Particle-In-Cell Modeling of Plasma-Based Accelerators in Two and Three Dimensions

In this dissertation, a fully object-oriented, fully relativistic, multi-dimensional Particle-In-Cell code was developed and applied to answer key questions in plasma-based accelerator research. The simulations increase the understanding of the processes in laser plasma and beam-plasma interaction, allow for comparison with experiments, and motivate the development of theoretical models. The simulations support the idea that the injection of electrons in a plasma wave by using a transversely propagating laser pulse is possible. The beam parameters of the injected electrons found in the simulations compare reasonably with beams produced by conventional methods and therefore laser injection is an interesting concept for future plasma-based accelerators. Simulations of the optical guiding of a laser wakefield driver in a parabolic plasma channel support the idea that electrons can be accelerated over distances much longer than the Rayleigh length in a channel. Simulations of plasma wakefield acceleration in the nonlinear blowout regime give a detailed picture of of the highly nonlinear processes involved. Using OSIRIS, we have also been able to perform full scale simulations of the E-157 experiment at the Stanford Linear Accelerator Center. These simulations have aided the experimentalists and they have assisted in the development of a theoretical model that is able to reproduce some important aspects of the full PIC simulations. Update (2015): This dissertation was originally written in 2000. I am making it now available on arXiv with the hope that some its content might proof useful to the users of the OSIRIS code which has continued to be utilized by a number of research groups since it was originally written as part of the research presented in this dissertation.

==> Cerenkov/cerenkov.tex <==
\chapter{3D Effects in the Generation of Cerenkov Wakes}
  \label{chap:cerenkov}



\section{Section1}
  \label{sect:cerenkov:section1} 
  
  


\section{Section2}
  \label{sect:cerenkov:section2}
  
  


\section{Section3}
  \label{sect:cerenkov:section3}  
  
  


\section{Conclusions}
  \label{sect:cerenkov:conclusions}



==> Osiris/os-modules.tex <==
\chapter{OSIRIS Modules}
  \label{chap:os-modules}
  
In its current form OSIRIS consists of 31 different modules. 23 of those
modules are classes in the sense of object oriented programing, that means
contain a type defintion and the methods acting
on variables of this type. The remaining 8 modules are containing subroutines or parameters
that are used by several of the other modules. In the module descriptions below the
prefixes "m\_" for module names and "t\_" for type names will be omitted when
this is possible without ambiguities.

\begin{description}

\item[m\_particles] This module defines the particle class. There is only one
particle object used in the code. It contains all information regarding the particles
in the simulation. It is composed of an arbitrary number of species objects
(including $0$ species objects) and an object of type diag\_particles. 
The definition of the type is:

%\begin{figure}
%   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_particles

!         allow access to type components only to module procedures
          private

!         number of species
          integer(p_k_is) :: num_species

!         diagnostics for all particles
          type( t_diag_particles )  ::  diag

!         pointer to array of species
          type( t_species ), dimension(:), pointer :: species

        end type t_particles

      \end{verbatim}
      }
%      \caption{The definition of the particle type in OSIRIS}
%      \label{fig:os-types:particles}
%   \end{center}
%\end{figure}

\item[m\_diag\_particles]

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_diag_particles

!         allow access to type components only to module procedures
          private

!         frequency of dumps
          integer(p_k_is)  ::    ndump_fac

!         file_name for data files
          character(80) :: file_name

!         variables to controle particle diagnostics
          logical            ::    if_particles_all
          real(p_k_rdoub)    ::    gamma_limit
          real(p_k_rdoub)    ::    particle_fraction

!         use of the following variables has not been implemented yet
          logical            ::    ifdmp_pa1
          integer(p_k_is)    ::    ndfrac_pa1
          logical            ::    ifdmp_pa2
          logical            ::    ifdmp_pa3
          real(p_k_rdoub)    ::    ndfrac_pa3
          logical            ::    ifdmp_dis

        end type t_diag_particles

      \end{verbatim}
      }
      \caption{The definition of the particle-diagnostic type in OSIRIS}
      \label{fig:os-types:diag-particles}
   \end{center}
\end{figure}

\item[m\_species]

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}
      
        type :: t_species

!         allow access to type components only to module procedures
          private

          integer(p_k_is) :: sp_id ! species-number - internal id

          integer(p_k_is) :: num_par_max ! max. # of part. for this species
          integer(p_k_is) :: num_par     ! actual number of particles

!         number of timesteps between sorting of particles
          integer(p_k_is) :: n_sort ! n_sort = 0 turns sorting off

!         general information for a species
          real(p_k_rdoub)                     :: rqm !  mass to charge ratio
!         # of part. in each direction in a grid cell
          integer(p_k_is), dimension(p_x_dim) :: num_par_x
          real(p_k_rdoub), dimension(p_p_dim) :: vth ! thermo-momentum
          real(p_k_rdoub), dimension(p_p_dim) :: vfl ! fluid-momentum
          real(p_k_rdoub)   :: den_min ! approx. min. density for a particle
          type( t_profile ) :: den ! inital density profile for this species

!         switch to turn off automatic neutralizing background
!         by solving Poissons equation in the beginning
          logical :: if_unneutralized ! this switch is currently deactivated

!         number of acceleration steps and increase in gamma at
!         at each step if the species is used as beam (in direction x1)
          real(p_k_rdoub) :: dgam
          integer(p_k_is) :: num_dgam

!         essential particle data position, momentum, and charge
          real(p_k_rdoub), dimension(:,:), pointer :: x, p
          real(p_k_rdoub), dimension(:),   pointer :: q

          type( t_spe_bound ) :: bnd_con ! boundary cond. for this species

          type( t_diag_species ) :: diag ! diagnostic for this species

        end type t_species

      \end{verbatim}
      }
      \caption{The definition of the species type in OSIRIS}
      \label{fig:os-types:species}
   \end{center}
\end{figure} 

\item[m\_diag\_species] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_diag_species

!         allow access to type components only to module procedures
          private

!         frequency of phasespace data dumps
          integer(p_k_is) :: ndump_fac_pha

!         file_name prefix for data files
          character(80) :: file_name

!         physical range for phasespace data dumps
          real(p_k_rdoub), dimension(p_x_dim) :: ps_xmin, ps_xmax
          real(p_k_rdoub), dimension(p_p_dim) :: ps_pmin, ps_pmax

!         resolutions for phasespace data dumps
          integer(p_k_is), dimension(p_x_dim) :: ps_nx
          integer(p_k_is), dimension(p_p_dim) :: ps_np

!         switches to turn on and off species phase space diagnostics
          logical :: if_x2x1, if_x3x1, if_p1x1, if_p2x1, if_p3x1
          logical ::          if_x3x2, if_p1x2, if_p2x2, if_p3x2
          logical ::                   if_p1x3, if_p2x3, if_p3x3
          logical ::                            if_p2p1, if_p3p1
          logical ::                                     if_p3p2

!         switches to turn on and off other species diagnostics
          logical :: iforigin, iftestpar ! currently not used

!         for diagnostic purposes : - currently not used
!         original position, momentum, and charge of particles
          real(p_k_rdoub), dimension(:,:), pointer :: xor, por
          real(p_k_rdoub), dimension(:),   pointer :: qor
!         particle identifier
          integer(p_k_is), dimension(:),   pointer :: pid

        end type t_diag_species

      \end{verbatim}
      }
      \caption{The definition of the species-diagnostic type in OSIRIS}
      \label{fig:os-types:diag-species}
   \end{center}
\end{figure}

\item[m\_spe\_bound] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_spe_bound

!         allow access to type components only to module procedures
          private

!         type of boundary conditions for each boundary
!         -1 : boundary to other node
!          0 : periodic b.c.
!          1 : boundary moving into the simulation box with c
!          2 : boundary moving outward from the simulation box with c
!          3 : not implemented yet - moving  inward (any velocity) ???
!          4 : not implemented yet - moving outward (any velocity) ???
!          5 : conducting boundary with particle absorption
!         20 : axial b.c. for cylindrical coordinates
!         30 : Lindman open-space boundary - limited implementation
!         indices: (lower-upper bound, direction)
          integer(p_k_is), dimension(2,p_x_dim) :: type

        end type t_spe_bound

      \end{verbatim}
      }
      \caption{The definition of the species-boundary type in OSIRIS}
      \label{fig:os-types:spe-bound}
   \end{center}
\end{figure} 

\item[m\_p\_status] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_p_status

!         allow access to type components only to module procedures
          private

          character :: data

!         The representaion of the status of a particle is given   
!         by a a byte character. The meaning of the differnt bits 
!         of the byte (bit 0 through 7) is : (if the bit is set)
!         0 : the particle will be removed from the simulation
!         1 : the particle moves out of the box through lower x1-bound.
!         2 : the particle moves out of the box through upper x1-bound.
!         3 : the particle moves out of the box through lower x2-bound.
!         4 : the particle moves out of the box through upper x2-bound.
!         5 : the particle moves out of the box through lower x3-bound.
!         6 : the particle moves out of the box through upper x3-bound.
!         7 : currently not implemented

        end type t_p_status

      \end{verbatim}
      }
      \caption{The definition of the particle-status type in OSIRIS}
      \label{fig:os-types:p-status}
   \end{center}
\end{figure}

\item[m\_profile] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_profile

!         allow access to type components only to module procedures
          private

!         number of points in profile
          integer(p_k_is) :: num_x

!         allocate later: x,fx( num_x, p_x_dim )
          real(p_k_rdoub), dimension(:,:), pointer :: x,fx

!         flag to center profile around a centroid
          logical                                  :: if_centroid

!         additional information required for centroid
!         allocate later: cent( num_x, p_x_dim )
!                         m, b( num_x-1, p_x_dim-1)
          real(p_k_rdoub), dimension(:,:), pointer :: cent,m,b

        end type t_profile

      \end{verbatim}
      }
      \caption{The definition of the profile type in OSIRIS}
      \label{fig:os-types:profile}
   \end{center}
\end{figure}

\item[m\_species\_utilities] test



\item[m\_el\_mag\_fld] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_el_mag_fld

!         allow access to type components only to module procedures
          private

!         electromagnetic field values on the grid:            
          type( t_vdf ) :: b, e

!         switches that influence how the field is calculated
          logical :: ifextfld, ifnotscon

!         initial external static magnetic and electric fields
          real(p_k_rdoub), dimension(p_f_dim) ::  b0, e0

!         boundary conditions for the electromagnetic field
          type( t_emf_bound )  ::  bnd_con

!         diagnostic set up for fields
          type( t_diag_emf ) :: diag

        end type t_el_mag_fld

      \end{verbatim}
      }
      \caption{The definition of the electromagnetic-field type in OSIRIS}
      \label{fig:os-types:el-mag-fld}
   \end{center}
\end{figure}

\item[m\_diag\_emf] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_diag_emf

!         allow access to type components only to module procedures
          private

!         frequency of dumps
          integer(p_k_is) ::    ndump_fac_all, ndump_fac_ave

!         file_name for data files
          character(80) :: file_name_all, file_name_ave

!         number of gridpoints to average over for averaged dumps
          integer(p_k_is), dimension(p_x_dim) :: n_ave

!         switches to decide which fields to write         
          logical, dimension(p_f_dim)  ::  ifdmp_efl
          logical, dimension(p_f_dim)  ::  ifdmp_bfl

!         switches between averaging and taking the envelope  
          logical, dimension(p_f_dim)  ::  ifenv_efl
          logical, dimension(p_f_dim)  ::  ifenv_bfl

!         switch to show initial static fields in data dumps
          logical                      ::  if_show_initial_fields

!         currently not implemented
          logical                      ::  ifdmp_s1f
          logical                      ::  ifdmp_dve
          logical                      ::  ifdmp_dvb
          logical                      ::  ifdmp_ede

        end type t_diag_emf

      \end{verbatim}
      }
      \caption{The definition of the electromagnetic-field-diagnostic
               type in OSIRIS}
      \label{fig:os-types:diag-emf}
   \end{center}
\end{figure}

\item[m\_emf\_bound] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_emf_bound

!         allow access to type components only to module procedures
          private

!         type of boundary conditions for each boundary
!         -1 : boundary to other node
!          0 : periodic b.c.
!          1 : boundary moving into the simulation box with c
!          2 : boundary moving outward from the simulation box with c
!          3 : not implemented yet - moving  inward (any velocity) ???
!          4 : not implemented yet - moving outward (any velocity) ???
!          5 : conducting boundary with particle absorption
!         20 : axial b.c. for cylindrical coordinates
!         30 : Lindman open-space boundary - limited implementation
!         indices: (lower-upper bound, direction)
          integer(p_k_is), dimension(2,p_x_dim) :: type

!         storrage for fields at boundaries at previous timestep
!         required for boundary conditions like lindman b.c.
!         note that currently only the memory for two oppsing
!         boundaries is implemented
!         lower boundary magnetic field
          real(p_k_rdoub), dimension(:,:),     pointer :: lbb_ptr1
          real(p_k_rdoub), dimension(:,:,:),   pointer :: lbb_ptr2
          real(p_k_rdoub), dimension(:,:,:,:), pointer :: lbb_ptr3
!         upper boundary magnetic field
          real(p_k_rdoub), dimension(:,:),     pointer :: ubb_ptr1
          real(p_k_rdoub), dimension(:,:,:),   pointer :: ubb_ptr2
          real(p_k_rdoub), dimension(:,:,:,:), pointer :: ubb_ptr3
!         lower boundary electric fields
          real(p_k_rdoub), dimension(:,:),     pointer :: lbe_ptr1
          real(p_k_rdoub), dimension(:,:,:),   pointer :: lbe_ptr2
          real(p_k_rdoub), dimension(:,:,:,:), pointer :: lbe_ptr3
!         upper boundary electric fields
          real(p_k_rdoub), dimension(:,:),     pointer :: ube_ptr1
          real(p_k_rdoub), dimension(:,:,:),   pointer :: ube_ptr2
          real(p_k_rdoub), dimension(:,:,:,:), pointer :: ube_ptr3

        end type t_emf_bound

      \end{verbatim}
      }
      \caption{The definition of the electromagnetic-field-boundary
               type in OSIRIS}
      \label{fig:os-types:emf-bound}
   \end{center}
\end{figure}



\item[m\_pulse\_sequence] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_pulse_sequence

!         allow access to type components only to module procedures
          private

!         number of pulses
          integer(p_k_is) :: num_pulses

!         pointer to array of pulses
          type (t_pulse), dimension(:), pointer :: pulse

        end type t_pulse_sequence
      \end{verbatim}
      }
      \caption{The definition of the pulse-sequence type in OSIRIS}
      \label{fig:os-types:pulse-sequence}
   \end{center}
\end{figure}

\item[m\_pulse] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_pulse
!         allow access to type components only to module procedures
          private
!         iflaunch: switch to turn on/off the pulse 
          logical :: iflaunch 
!         wavetype:  type/direction of pulse to be launched
!                  1->x1, 2->x2
          integer(p_k_is) :: wavetype  
!         size of the pulse 
!         w0:     focal spotsize
!         rise:   the length for the pulse to rise from zero to peak
!         fall:   length for the pulse to fall to zero
!         length: length of the peak part
!          real(p_k_rdoub), dimension( p_x_dim - 1 ) :: w0
          real(p_k_rdoub) :: w0
          real(p_k_rdoub) :: rise, fall, length
!         laser light properties
!         vosc:   maximum normalized vectorpotential of laser
!         rkkp:   k-number of laser in normalized units
!         pol:    polarization
!         phase:  global phaseshift
          real(p_k_rdoub) :: vosc, rkkp, pol, phase
!         position and time of pulse launch
!         start:  location of pulse front at setup of pulse
!                 measured from the boundary the pulse is
!                 propagating towards
!         focus:  location of focal point of the pulse
!                 measured the same way as start
!         offset: offset of pulse center from center of simulation
!                 box; positive -> shift to the right of propagation
!                 (in 2D), negative -> shift to the left (in 2D)
!         time:   time at which the pulse is to be initialized
          real(p_k_rdoub)                         :: start
!          real(p_k_rdoub), dimension(p_x_dim - 1) :: focus
          real(p_k_rdoub)                         :: focus
          real(p_k_rdoub), dimension(p_x_dim - 1) :: offset
          real(p_k_rdoub)                         :: time
        end type t_pulse

      \end{verbatim}
      }
      \caption{The definition of the pulse type in OSIRIS}
      \label{fig:os-types:pulse}
   \end{center}
\end{figure}


\item[m\_phy\_field] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_phy_field

!         allow access to type components only to module procedures
          private

!         physical field data
!         (source field - current, charge density)
          type( t_vdf ) :: pf

!         boundary conditions 
          type( t_phy_field_bound )  ::  bnd_con

!         definition of smoothing 
          type( t_smooth )  ::  smooth

!         diagnostic setup  
          type( t_diag_phy_field ) :: diag

        end type t_phy_field

      \end{verbatim}
      }
      \caption{The definition of the source-field type in OSIRIS. Note that
               source-fields are referred to in the code as physical fields}
      \label{fig:os-types:phy-field}
   \end{center}
\end{figure}

\item[m\_diag\_phy\_field] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_diag_phy_field

!         allow access to type components only to module procedures
          private

!         frequency of data dumps
          integer(p_k_is) :: ndump_fac_all, ndump_fac_ave

!         file name for data files
          character(80) :: file_name_all, file_name_ave

!         number of gridpoints to average over for averaged data
          integer(p_k_is), dimension(p_x_dim) :: n_ave
 
!         switches for turning on and off the different field components        
          logical, dimension(p_f_dim) :: ifdmp_phy_field  

!         variables to set whether the average or the envelope
!         of the field is taken for the average field dumps
          logical, dimension(p_f_dim) :: ifenv_phy_field

        end type t_diag_phy_field

      \end{verbatim}
      }
      \caption{The definition of the source-field-diagnostic type in OSIRIS}
      \label{fig:os-types:diag-phy-field}
   \end{center}
\end{figure}

\item[m\_phy\_field\_bound] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_phy_field_bound

!         allow access to type components only to module procedures
          private

!         type of boundary conditions for each boundary
!         -1 : boundary to other node
!          0 : periodic b.c.
!          1 : boundary moving into the simulation box with c
!          2 : boundary moving outward from the simulation box with c
!          3 : not implemented yet - moving  inward (any velocity) ???
!          4 : not implemented yet - moving outward (any velocity) ???
!          5 : conducting boundary with particle absorption
!         20 : axial b.c. for cylindrical coordinates
!         30 : Lindman open-space boundary - limited implementation
!         indices: (lower-upper bound, direction)
          integer(p_k_is), dimension( 2 , p_x_dim ) :: type

        end type t_phy_field_bound

      \end{verbatim}
      }
      \caption{The definition of the source-field-boundary type in OSIRIS}
      \label{fig:os-types:phy-field-bound}
   \end{center}
\end{figure}

\item[m\_smooth] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_smooth

!         allow access to type components only to module procedures
          private

!         switches for smoothing in each direction
          logical, dimension(p_x_dim)  ::  ifsmooth

!         level of smoothing (number of neighboring cells included)
          integer(p_k_is), dimension(p_x_dim)  ::  smooth_level, nsm

!         smoothing weighting factors of each successive smoothing
!         step for the field in x(:) - these are given in the input dec
!         swfj( 1:3 , maxval(nsm), p_x_dim )
          real(p_k_rdoub), dimension(:,:,:), pointer :: swfj

!         coefficients of the one step smoothing calculated from swfj
!         scoef( maxval(nscoef)+1, p_x_dim )
          real(p_k_rdoub), dimension(:,:), pointer :: scoef

!         number of smoothing coefficients in each direction
!         nscoef(i) = 2*nsm(i)+1
          integer(p_k_is), dimension(p_x_dim) ::  nscoef

        end type t_smooth

      \end{verbatim}
      }
      \caption{The definition of the smooth type in OSIRIS}
      \label{fig:os-types:smooth}
   \end{center}
\end{figure}


\item[m\_node\_conf] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_node_conf

!         allow access to type components only to module procedures
          private

!         total number of nodes
          integer(p_k_is) :: no_num

!         number of nodes in each dimension
          integer(p_k_is), dimension(p_x_dim) :: nx

!         array identification number of this node
!         (this is the location in the task-id-array (tid) )
          integer(p_k_is) :: my_aid

!         N_ode G_rid P_osition
!         (within the grid of nodes given by [nx(1),nx(2),nx(3)] )
          integer(p_k_is), dimension(p_x_dim) :: my_ngp

!         array identification number of neighboring nodes
!         (this will probably be useless for dynamic load balancing)
          integer(p_k_is), dimension( 2, p_x_dim ) :: neighbor

!         flags for periodic node grid (periodic boundary conditions)
          logical, dimension(p_x_dim) :: ifpr

!         total extent of system in each direction
!         needed for particle communication along periodic directions
!         the information has to be updated from global space
          real(p_k_rdoub), dimension(p_x_dim) :: x_extent

!         task ids of all "no_num" processes
          integer(p_k_is), dimension(:), pointer :: tid

        end type t_node_conf

      \end{verbatim}
      }
      \caption{The definition of the node-configuration type in OSIRIS}
      \label{fig:os-types:node-conf}
   \end{center}
\end{figure}

\item[m\_vdf] test

Fig.~\ref{fig:os-algorithms:vdf-type}

%\begin{figure}
%   \begin{center}
%      \small{
%      \begin{verbatim}
%
%        type :: t_vdf
%
%!         allow access to type components only to module procedures
%          private
%
%!         variable to indicate status of vdf-object
%          logical :: associated
%
%!         pointer to field data for field 1D space f(j,i1)
%          real(p_k_rdoub), dimension(:,:), pointer :: f1
%
%!         pointer to field data for field 2D space f(j,i1,i2)
%          real(p_k_rdoub), dimension(:,:,:), pointer :: f2
%
%!         pointer to field data for field 3D space f(j,i1,i2,i3)
%          real(p_k_rdoub), dimension(:,:,:,:), pointer :: f3
%
%!         grid information for this object on the local node
%          type( t_grid ), pointer :: grid
%
%        end type t_vdf
%
%      \end{verbatim}
%      }
%      \caption{The definition of the VDF-type in OSIRIS}
%      \label{fig:os-types:vdf}
%   \end{center}
%\end{figure}

\item[m\_grid] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_grid
!         allow access to type components only to module procedures
          private
          integer(p_k_is), dimension(p_x_dim) :: nx_p ! gridsize
!         boundary values of grid counter (position of this grid
!         relative to the initial global grid with respect to which
!         this grid - whether global or local - was setup originally)
          integer(p_k_is), dimension(p_x_dim) :: nx_p_min, nx_p_max
!         number of guard cells at the boundaries, the physical range
!         of the field is from 1 to (max - upper_gc) for each direction
!         indices: (lower-upper bound, direction)
          integer(p_k_is), dimension(:,:), pointer :: gc_num
!         switches that turn on and off whether gc_num is checked
!         for compatibility with the grid when it is changed
          logical, dimension(p_x_dim) :: if_check_gc
!         location of field values in grid cell - not used currently
!         allocation: dimension(x_dim,# of components of field)
          real(p_k_rdoub), dimension(:,:), pointer :: odx
!         size of gridcell, its reciprocal value, and a number that can
!         be used to implement a tolerance of grid point positions
!         against numerical error
          real(p_k_rdoub), dimension(p_x_dim) :: dx, rdx, dx_tol
!         variable to select the type of coordinates for the space
!         currently implemented coordinate systems:
!         coordinates = p_cartesian      : carthesian corrdinates
!         coordinates = p_cylindrical_b  : cyl. coordinates B1 on axis
!         coordinates = p_cylindrical_e  : cyl. coordinates E1 on axis
!                                        (symmetric if in 2D)
!         other possible implementations: polar(in 2D), spherical
          integer(p_k_is) :: coordinates
!         radii and their inv. given at corner and the middle of cells
          real(p_k_rdoub), dimension(:), pointer ::  rad_cor,  rad_mid
          real(p_k_rdoub), dimension(:), pointer :: rrad_cor, rrad_mid
        end type t_grid

      \end{verbatim}
      }
      \caption{The definition of the grid type in OSIRIS}
      \label{fig:os-types:grid}
   \end{center}
\end{figure}

\item[m\_space] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_space

!         allow access to type components only to module procedures
          private

!         first general information on the simulation box that
!         is independent on how the boundaries of the box move
!         over longer periods of time

!         space in simulation box
          real(p_k_rdoub), dimension(2,p_x_dim) :: x_bnd

!         space in simulation box before last call of
!         move_boundary
          real(p_k_rdoub), dimension(2,p_x_dim) :: x_bnd_old

!         number of dx the boundaries of the space move at
!         current timestep
!         the sign indicates the direction of the motion of
!         each boundary
          integer(p_k_is), dimension(2,p_x_dim) :: move_num

!         distances moved since last move of space boundaries
          real(p_k_rdoub), dimension(2,p_x_dim) :: xmoved

!         the following variable(s) contain information about
!         the specific motion of the simulation box
!         at this time only motion with c is implemented

!         information on motion of the simulation box
          logical, dimension(p_x_dim) :: if_move

        end type t_space

      \end{verbatim}
      }
      \caption{The definition of the space type in OSIRIS}
      \label{fig:os-types:space}
   \end{center}
\end{figure}

\item[m\_time\_step] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_time_step

!         allow access to type components only to module procedures
          private

          real(p_k_rdoub) :: dt    ! timestep length
          integer(p_k_is) :: n     ! timestep counter
          integer(p_k_is) :: ndump ! "master" timestep
                                   ! for reports/data dumps
        end type t_time_step

      \end{verbatim}
      }
      \caption{The definition of the time-step type in OSIRIS}
      \label{fig:os-types:time-step}
   \end{center}
\end{figure}

\item[m\_time] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_time

!         allow access to type components only to module procedures
          private

          real(p_k_rdoub) :: tmin, tmax, t

        end type t_time

      \end{verbatim}
      }
      \caption{The definition of the time type in OSIRIS}
      \label{fig:os-types:time}
   \end{center}
\end{figure}


\item[m\_restart] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

        type :: t_restart

!         allow access to type components only to module procedures
          private

!         frequency of restart dumps
          integer(p_k_is)  ::  ndump_fac

!         file name for  restart files
          character(80) :: file_name

!         switch to restart from a restart file
          logical   ::   if_restart

        end type t_restart

      \end{verbatim}
      }
      \caption{The definition of the restart type in OSIRIS}
      \label{fig:os-types:restart}
   \end{center}
\end{figure}

\item[m\_diagnostic\_utilities] test

\item[m\_utilities] test

\item[m\_file\_system] test

\item[m\_units] test

\item[m\_parameters] test

\begin{figure}
   \begin{center}
      \small{
      \begin{verbatim}

!==============================================================
!       parameters essential at compile time
!~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

!       define parameters describing the physics of the simulation
        integer(p_k_is), parameter :: p_x_dim=3 !no. of dim. of space
        integer(p_k_is), parameter :: p_p_dim=3 !no. of dim. of momentum
        integer(p_k_is), parameter :: p_f_dim=3 !no. of comp. of a vectorfield

!==============================================================
!       parameters to identify coordinate systems
!~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

        integer(p_k_is), parameter :: p_cartesian     = 0
        integer(p_k_is), parameter :: p_cylindrical_b = 1 ! B1 on axis
        integer(p_k_is), parameter :: p_cylindrical_e = 2 ! E1 on axis
        integer(p_k_is), parameter :: p_polar_2d      = 3
        integer(p_k_is), parameter :: p_spherical     = 4

      \end{verbatim}
      }
      \caption{The fundamental parameters used in OSIRIS.}
      \label{fig:os-types:parameters}
   \end{center}
\end{figure}

\item[m\_system] test

\item[m\_mpi\_replacement] test

\end{description}



==> Osiris/os-performance.tex <==
\chapter{The computational performance of OSIRIS}
  \label{chap:os-performance}



\section{Section1}
  \label{sect:os-performance:section1} 
  
  


\section{Section2}
  \label{sect:os-performance:section2}
  
  


\section{Section3}
  \label{sect:os-performance:section3}  
  
  


\section{Summary}
  \label{sect:os-performance:summary}


